DA-VSR: Domain Adaptable Volumetric Super-Resolution For Medical Images

Medical image super-resolution (SR) is an active research area that has many potential applications, including reducing scan time, bettering visual understanding, increasing robustness in downstream tasks, etc. However, applying deep-learning-based SR approaches for clinical applications often encounters issues of domain inconsistency, as the test data may be acquired by different machines or on different organs. In this work, we present a novel algorithm called domain adaptable volumetric super-resolution (DA-VSR) to better bridge the domain inconsistency gap. DA-VSR uses a unified feature extraction backbone and a series of network heads to improve image quality over different planes. Furthermore, DA-VSR leverages the in-plane and through-plane resolution differences on the test data to achieve a self-learned domain adaptation. As such, DA-VSR combines the advantages of a strong feature generator learned through supervised training and the ability to tune to the idiosyncrasies of the test volumes through unsupervised learning. Through experiments, we demonstrate that DA-VSR significantly improves super-resolution quality across numerous datasets of different domains, thereby taking a further step toward real clinical applications.

==> images/backup_subfloat.tex <==
\begin{figure}[!t]
	\scriptsize
    \begin{tabular}[b]{cc}
        \subfloat[][hello.]{5pt}
        {
            \includegraphics[width=\linewidth,height=0.6\linewidth,cframe=red]{images/case3/gt_134_hr_box.png}
        % \caption*{\stackanchor{Case 1}{}}
        }
        &
        \begin{tabular}[b]{c c c c}
            \subfloat[][b]%{0.15\linewidth}
            {
                \setlength{\abovecaptionskip}{3pt}
                \includegraphics[width=\linewidth,height=0.5\linewidth,cframe=red]{images/case3/gt.png}
                % \caption*{\stackanchor{$\textrm{HR}_{}$}{PSNR/SSIM}}
            % \end{subfloat}
            }
            &
            \subfloat[][b]%{0.15\linewidth}
            {
                \setlength{\abovecaptionskip}{3pt}
                \includegraphics[width=\linewidth,height=0.5\linewidth,cframe=red]{images/case3/gt.png}
                % \caption*{\stackanchor{$\textrm{HR}_{}$}{PSNR/SSIM}}
            % \end{subfloat}
            }
            &
            \subfloat[][b]%{0.15\linewidth}
            {
                \setlength{\abovecaptionskip}{3pt}
                \includegraphics[width=\linewidth,height=0.5\linewidth,cframe=red]{images/case3/gt.png}
                % \caption*{\stackanchor{$\textrm{HR}_{}$}{PSNR/SSIM}}
            % \end{subfloat}
            }
            &
            \subfloat[][b]%{0.15\linewidth}
            {
                \setlength{\abovecaptionskip}{3pt}
                \includegraphics[width=\linewidth,height=0.5\linewidth,cframe=red]{images/case3/gt.png}
                % \caption*{\stackanchor{$\textrm{HR}_{}$}{PSNR/SSIM}}
            % \end{subfloat}
            }\\
            \subfloat[][b]%{0.15\linewidth}
            {
                \setlength{\abovecaptionskip}{3pt}
                \includegraphics[width=\linewidth,height=0.5\linewidth,cframe=red]{images/case3/gt.png}
                % \caption*{\stackanchor{$\textrm{HR}_{}$}{PSNR/SSIM}}
            % \end{subfloat}
            }
            &
            \subfloat[][b]%{0.15\linewidth}
            {
                \setlength{\abovecaptionskip}{3pt}
                \includegraphics[width=\linewidth,height=0.5\linewidth,cframe=red]{images/case3/gt.png}
                % \caption*{\stackanchor{$\textrm{HR}_{}$}{PSNR/SSIM}}
            % \end{subfloat}
            }
            &
            \subfloat[][b]%{0.15\linewidth}
            {
                \setlength{\abovecaptionskip}{3pt}
                \includegraphics[width=\linewidth,height=0.5\linewidth,cframe=red]{images/case3/gt.png}
                % \caption*{\stackanchor{$\textrm{HR}_{}$}{PSNR/SSIM}}
            % \end{subfloat}
            }
            &
            \subfloat[][b]%{0.15\linewidth}
            {
                \setlength{\abovecaptionskip}{3pt}
                \includegraphics[width=\linewidth,height=0.5\linewidth,cframe=red]{images/case3/gt.png}
                % \caption*{\stackanchor{$\textrm{HR}_{}$}{PSNR/SSIM}}
            % \end{subfloat}
            }
        \end{tabular}
    \end{tabular}\\
    % \begin{tabular}[b]{cc}
    %     \begin{subfloat}[b]{0.38\linewidth}
    %         \includegraphics[width=\linewidth,height=0.6\linewidth,cframe=red]{images/vis/gt_111_box.png}
    %     \caption*{\stackanchor{Case 2}{}}
    %     \end{subfloat}
    %     &
    %     \begin{tabular}[b]{c c c c}
    %         \begin{subfloat}[b]{0.15\linewidth}
    %             \setlength{\abovecaptionskip}{3pt}
    %             \includegraphics[width=\linewidth,height=0.5\linewidth,cframe=red]{images/case2/gt_111_patch.png}
    %             \caption*{\stackanchor{$\textrm{HR}_{}$}{PSNR/SSIM}}
    %         \end{subfloat}
    %         &
    %         \begin{subfloat}[b]{0.15\linewidth}
    %             \setlength{\abovecaptionskip}{3pt}
    %             \includegraphics[width=\linewidth,height=0.5\linewidth,cframe=red]{images/case2/ref_111_patch.png}
    %             \caption*{\stackanchor{$\textrm{DA-VSR}_{}$}{\bf{34.91/0.980}}}
    %         \end{subfloat}
    %         &
    %         \begin{subfloat}[b]{0.15\linewidth}
    %             \setlength{\abovecaptionskip}{3pt}
    %             \includegraphics[width=\linewidth,height=0.5\linewidth,cframe=red]{images/case2/no_ref_111_patch.png}
    %             \caption*{\stackanchor{$\textrm{DA-VSR}_{NA}$}{34.78/0.976}}
    %         \end{subfloat}
    %         &
    %         \begin{subfloat}[b]{0.15\linewidth}
    %             \setlength{\abovecaptionskip}{3pt}
    %             \includegraphics[width=\linewidth,height=0.5\linewidth,cframe=red]{images/case2/saint_111_patch.png}
    %             \caption*{\stackanchor{$\textrm{SAINT}_{}$}{34.84/0.977}}
    %         \end{subfloat}\\
    %         \begin{subfloat}[b]{0.15\linewidth}
    %             \setlength{\abovecaptionskip}{3pt}
    %             \includegraphics[width=\linewidth,height=0.5\linewidth,cframe=red]{images/case2/smore_111_patch.png}
    %             \caption*{\stackanchor{SMORE}{34.65/0.978}}
    %         \end{subfloat}
    %         &
    %         \begin{subfloat}[b]{0.15\linewidth}
    %             \setlength{\abovecaptionskip}{3pt}
    %             \includegraphics[width=\linewidth,height=0.5\linewidth,cframe=red]{images/case2/rdn_111_patch.png}
    %             \caption*{\stackanchor{3DRDN}{34.47/0.966}}
    %         \end{subfloat}
    %         &
    %         \begin{subfloat}[b]{0.15\linewidth}
    %             \setlength{\abovecaptionskip}{3pt}
    %             \includegraphics[width=\linewidth,height=0.5\linewidth,cframe=red]{images/case2/rcan_111_patch.png}
    %             \caption*{\stackanchor{3DRCAN}{34.60/0.965}}
    %         \end{subfloat}
    %         &
    %         \begin{subfloat}[b]{0.15\linewidth}
    %             \setlength{\abovecaptionskip}{3pt}
    %             \includegraphics[width=\linewidth,height=0.5\linewidth,cframe=red]{images/case2/cubic_111_patch.png}
    %             \caption*{\stackanchor{Bicubic}{31.60/0.926}}
    %         \end{subfloat}
    %     \end{tabular}
    % \end{tabular}    \\
    % \begin{tabular}[b]{cc}
    %     \begin{subfloat}[b]{0.38\linewidth}
    %         \includegraphics[width=\linewidth,height=0.6\linewidth,cframe=red]{images/vis/gt_box.png}
    %     \caption*{\stackanchor{Case 3}{}}
    %     \end{subfloat}
    %     &
    %     \begin{tabular}[b]{c c c c}
    %         \begin{subfloat}[b]{0.15\linewidth}
    %             \setlength{\abovecaptionskip}{3pt}
    %             \includegraphics[width=\linewidth,height=0.5\linewidth,cframe=red]{images/vis/gt_026_patch.png}
    %             \caption*{\stackanchor{$\textrm{HR}_{}$}{PSNR/SSIM}}
    %         \end{subfloat}
    %         &
    %         \begin{subfloat}[b]{0.15\linewidth}
    %             \setlength{\abovecaptionskip}{3pt}
    %             \includegraphics[width=\linewidth,height=0.5\linewidth,cframe=red]{images/vis/ref_026_patch.png}
    %             \caption*{\stackanchor{$\textrm{DA-VSR}_{}$}{\bf{37.83/0.978}}}
    %         \end{subfloat}
    %         &
    %         \begin{subfloat}[b]{0.15\linewidth}
    %             \setlength{\abovecaptionskip}{3pt}
    %             \includegraphics[width=\linewidth,height=0.5\linewidth,cframe=red]{images/vis/no_ref_026_patch.png}
    %             \caption*{\stackanchor{$\textrm{DA-VSR}_{NA}$}{36.68/0.969}}
    %         \end{subfloat}
    %         &
    %         \begin{subfloat}[b]{0.15\linewidth}
    %             \setlength{\abovecaptionskip}{3pt}
    %             \includegraphics[width=\linewidth,height=0.5\linewidth,cframe=red]{images/vis/saint_026_patch.png}
    %             \caption*{\stackanchor{$\textrm{SAINT}_{}$}{36.77/0.969}}
    %         \end{subfloat}\\
    %         \begin{subfloat}[b]{0.15\linewidth}
    %             \setlength{\abovecaptionskip}{3pt}
    %             \includegraphics[width=\linewidth,height=0.5\linewidth,cframe=red]{images/vis/smore_026_patch.png}
    %             \caption*{\stackanchor{SMORE}{35.08/0.954}}
    %         \end{subfloat}
    %         &
    %         \begin{subfloat}[b]{0.15\linewidth}
    %             \setlength{\abovecaptionskip}{3pt}
    %             \includegraphics[width=\linewidth,height=0.5\linewidth,cframe=red]{images/vis/rdn_026_patch.png}
    %             \caption*{\stackanchor{3DRDN}{36.50/0.968}}
    %         \end{subfloat}
    %         &
    %         \begin{subfloat}[b]{0.15\linewidth}
    %             \setlength{\abovecaptionskip}{3pt}
    %             \includegraphics[width=\linewidth,height=0.5\linewidth,cframe=red]{images/vis/rcan_026_patch.png}
    %             \caption*{\stackanchor{3DRCAN}{36.42/0.967}}
    %         \end{subfloat}
    %         &
    %         \begin{subfloat}[b]{0.15\linewidth}
    %             \setlength{\abovecaptionskip}{3pt}
    %             \includegraphics[width=\linewidth,height=0.5\linewidth,cframe=red]{images/vis/bicub_026_patch.png}
    %             \caption*{\stackanchor{Bicubic}{31.62/0.927}}
    %         \end{subfloat}
    %     \end{tabular}
    % \end{tabular}       
    \caption{Visual comparisons of DA-VSR and other state-of-the-art implementations from the sagittal plane, highlight regions are contrast-adjusted. Case 1 is from the Colon dataset, Case 2 and 3 are from the Kidney dataset\cite{1904.00445}. In particular, Case 3 is a lung region cropped from a kidney-containing image. Please refer to the supplemental material for more visual comparisons.} 
    \label{fig:ablation_visual}
    \vspace{-1em}
\end{figure}
